Auditing and Enforcing Conditional Fairness via Optimal Transport

Conditional demographic parity (CDP) is a measure of the demographic parity of a predictive model or decision process when conditioning on an additional feature or set of features. Many algorithmic fairness techniques exist to target demographic parity, but CDP is much harder to achieve, particularly when the conditioning variable has many levels and/or when the model outputs are continuous. The problem of auditing and enforcing CDP is understudied in the literature. In light of this, we propose novel measures of {conditional demographic disparity (CDD)} which rely on statistical distances borrowed from the optimal transport literature. We further design and evaluate regularization-based approaches based on these CDD measures. Our methods, \fairbit{} and \fairlp{}, allow us to target CDP even when the conditioning variable has many levels. When model outputs are continuous, our methods target full equality of the conditional distributions, unlike other methods that only consider first moments or related proxy quantities. We validate the efficacy of our approaches on real-world datasets.

==> Xu_2021.tex <==
In \cite{xu2020algorithmic}, they propose a novel Derivable Conditional Fairness Regularizer (DCFR) to optimize conditional fairness by learning conditional independent representation. In their paper they propose the following regularizer 
\begin{align}
    L_{\text{fair}} (Z,L,A) := \sup_{h} Q(h) := \sup_{h} \left(\E[\mathbf{1}_{\{A=1\}}\Prob(A=0|L)h(Z,L)]- \E[\mathbf{1}_{\{A=0\}}\Prob(A=1|L)h(Z,L)]\right)
\end{align}
where $Z$ is a random variable (it is the f(X) in our setting). $h(Z,L)$ is a $L^2$ function on $Z, L$ space. Indeed, $Q(h)=0$ implies the conditional independence $Z\indep A | L$. However, we want to argue that by minimizing $Q(h)$ doesn't realize the CDP. More precisely,
\begin{align*}
     Q(h) &= \E[\mathbf{1}_{\{A=1\}}\Prob(A=0|L)h(Z,L)]- \E[\mathbf{1}_{\{A=0\}}\Prob(A=1|L)h(Z,L)]\\
     & =\E\left[\left(\mathbf{1}_{\{A=1\}}\Prob(A=0|L)- \mathbf{1}_{\{A=0\}}\Prob(A=1|L)\right)h(Z,L) \right]\\
     & =\E\left[\E\left[\mathbf{1}_{\{A=1\}}\Prob(A=0|L)- \mathbf{1}_{\{A=0\}}\Prob(A=1|L)|Z,L\right]h(Z,L) \right]  \\
     & =\E\left[ \underbrace{\left(\Prob(A=1|Z,L)\Prob(A=0|L)- \Prob(A=0|Z,L)\Prob(A=1|L)\right)}_{g(Z,L)}h(Z,L)\right]\\
     \Rightarrow  h(Z,L) &= \mathbf{1}_{\{g>0\}}\\
     & = \mathbf{1}_{\{\Prob(A=1|Z,L)\Prob(A=0|L)- \Prob(A=0|Z,L)\Prob(A=1|L)>0\}}\\
      & = \mathbf{1}_{\{  \frac{\Prob(A=1|Z,L)}{\Prob(A=1|L)} >\frac{\Prob(A=0|Z,L)}{\Prob(A=0|L)} \}}\\
      & = \mathbf{1}_{\{ \Prob(A=1|Z,L)>\Prob(A=1|L)\}}\\
      \Rightarrow  Q(h) &= \E[\left(\Prob(A=1|Z,L)\Prob(A=0|L)- \Prob(A=0|Z,L)\Prob(A=1|L)\right)_+]\\
      &=\E[ ( \Prob(A=1|Z,L)-\Prob(A=1|L) )_+ ]
\end{align*}
Take a simple example to illustrate the difference between $Q(h)$ and CDP. Let $L$ to be the level of income, for people with the same level of income, as shown in the following table, 
\begin{table}[h]
\centering
\resizebox{0.2\textwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
        & Male & Female \\ \midrule
Accept  & a & b \\
Decline & c & d \\ \bottomrule
\end{tabular}%
}
\end{table}

where CDP wants to minimize $\frac{a}{a+c}-\frac{b}{b+d}$, that is the accept rate for both male and female with the same level of income should be same, while $Q(h)$ represents $\frac{a}{a+b}-\frac{c}{c+d}$, that is to minimize the difference between the ratio of man in the approved people and the ratio of man in the whole candidate.

Figure \ref{fig:res:Xucomp_simple_example} provides a pictorial explanation, using a simulated population of $10,000$ individuals. We consider two parameters $p$ and $\delta$: $p$ is the proportion of female:male in the simulated data and $\delta$ controls the disparity in acceptance rates:

$$
P(\text{Accept} | \text{Male}) = 0.5 + \delta \quad, \quad  P(\text{Accept} | \text{Female}) = 0.5 - \delta.
$$


Figure \ref{fig:res:Xucomp_simple_example} (left) below shows that a small value of $Q(h)$ does not necessarily lead to a small conditional demographic disparity (CDD), as the relationship between these two quantities depends on the ratio of males to females in the underlying data. Different acceptance rates lead to various levels of CDD and $Q(h)$ values; the proportion of females controls the slope of this CDD-$Q(h)$ curve. More specifically, the fewer the females, the higher the CDD-$Q(h)$ slope, meaning a smaller value of $Q(h)$ would correspond to a much higher CDD. A 1:1 relationship (i.e., a slope of $1$) only happens if the ratio of females to male is 1:1. Figure \ref{fig:res:Xucomp_simple_example} (right) show that our proposed regularizer enjoys a practically 1:1 relationship with CDD, with some variance due to the finite sample, regardless of female:male proportion in the original data.

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/simple_example_xu/cdd_qh_plot_10k.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/simple_example_xu/cdd_fairbit_plot_10k.pdf}
    \end{minipage}
    \caption{\textit{Left}: $Q(h)$ versus conditional demographic disparity (CDD), varying the proportion of females and the acceptance rate of male vs. female in the simple example. Different acceptance rates lead to various levels of CDD and $Q(h)$ values; the proportion of females controls the slope of this CDD-$Q(h)$ curve. More specifically, the fewer the females, the higher the CDD-$Q(h)$ slope, meaning a smaller value of $Q(h)$ would correspond to a much higher CDD. A 1:1 relationship (i.e., a slope of $1$) only happens if the ratio of females to male is 1:1.  }
    \label{fig:res:Xucomp_simple_example}
\end{figure}

==> additional_numerical.tex <==

\luhao{Cross Entropy, Reg: f(x), Unfairness: f(x), ACC: 4 measures of accuracy}
\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-AUC-diff/conditional_statistical_parity_l1-accuracy.png}
        % \caption{$dt=0.1$}
        % \label{fig:loan:SP}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-AUC-diff/conditional_statistical_parity_l1-AUROC.png}
        % \caption{$dt =$}
        % \label{fig:loan:CSP1}
    \end{minipage}
\end{figure}
\begin{figure}    
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-AUC-diff/conditional_statistical_parity_l1-cross_entropy.png}
        % \caption{$dt=0.1$}
        % \label{fig:loan:CSP2}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-AUC-diff/conditional_statistical_parity_l1-MSE.png}
        % \caption{$dt =$}
        % \label{fig:loan:CSPI}
    \end{minipage}
    \caption{Demonstration of the trade-off between different measures of accuracy and fairness (CSP-$\ell_1$).}
    % \label{fig:loan:CSP}
\end{figure}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-iter/CSP_Infinity-5.png}
        % \caption{Bi-causal}
        % \label{fig:loan:SP}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-iter/CSP_Infinity-2.png}
        % \label{fig:loan:CSP1}
    \end{minipage}
    \caption{Demonstration of $\mathsf{CSP}_f^{\infty}$ (right) for each iterations as $\lambda$ changes for Bi-causal(left) and Sinkhorn (right), training with gradient descent.}
\end{figure}
\begin{figure}[!htb]
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-iter/CSP_Infinity-3.png}
        % \caption{Bi-causal with batches}
        % \label{fig:loan:CSP2}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-iter/CSP_Infinity-4.png}
        % \caption{Energy distance with batches}
        % \label{fig:loan:CSPI}
    \end{minipage}
    \caption{Demonstration of $\mathsf{CSP}_f^{\infty}$ (right) for each iterations as $\lambda$ changes for Bi-causal(left) and Energy distance (right), training with stochastic gradient descent with batch size $1000$.}
    % \label{fig:loan:CSP}
\end{figure}

\newpage
\luhao{Cross Entropy, Reg: f(x), Unfairness: f(x), ACC: 4 measures of accuracy, $X=\varepsilon_1+\varepsilon_2$ where $\varepsilon_1 \sim Uniform (0,5)$, $\varepsilon_2 \sim \mathcal N (0, 0.1 \exp(A))$}

\begin{figure}[!htb]
    \centering
    \begin{minipage}{.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/conditional_statistical_parity_l1-accuracy.png}
        % \caption{Bi-causal}
        % \label{fig:loan:SP}
    \end{minipage}%
    \begin{minipage}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/conditional_statistical_parity_l2-accuracy.png}
        % \label{fig:loan:CSP1}
    \end{minipage}
    \begin{minipage}{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/conditional_statistical_parity_linfty-accuracy.png}
        % \label{fig:loan:CSP1}
    \end{minipage}
    \caption{Demonstration of the trade-off between measures of accuracy rate and fairness.}
\end{figure}

\luhao{Another set of experiments with same setups}
\begin{figure}[!htb]
    \centering
    \begin{minipage}{.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/1-conditional_statistical_parity_l1-accuracy.png}
    \end{minipage}%
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/1-conditional_statistical_parity_l2-accuracy.png}
    \end{minipage}
\end{figure}
\begin{figure}[!htb]
\centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/1-conditional_statistical_parity_linfty-accuracy.png}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/loan-cov/1-statistical_parity-accuracy.png}
    \end{minipage}
    \caption{Demonstration of the trade-off between measures of accuracy rate and fairness.}
\end{figure}

==> baselines.tex <==
The current state of the art for CDP is the approach proposed in \cite{xu2020algorithmic}. This method, named Derivable Conditional Fairness Regularizer (DCFR), proposes the following regularizer to impose CDP by learning conditional independent representation:
\begin{align}
    R_{\text{DCFR}} (f(X),L,A) := \sup_{h} Q(h) := \sup_{h} \left(\E[\mathbf{1}_{\{A=1\}}\Prob(A=0|L)h(f(X),L)]- \E[\mathbf{1}_{\{A=0\}}\Prob(A=1|L)h(f(X),L)]\right),
\end{align}
where $h(Z,L)$ is a bounded $L^2$ function with values in $[0,1]$. As shown in \cite{daudin1980partial}, $Q(h)=0$ implies the conditional independence $Z\indep A | L$. However, Proposition~\ref{prop:dcfr_alternative_form} shows that $R_{\text{DCFR}}$ does not minimize CDP directly, but rather targets a related proxy quantity. This is in contrast with our proposed \bcd{}, which targets directly CDP
(see Proposition XXX \nic{Insert proposition for the one-liner upper bound in Section above.})

\begin{proposition}\label{prop:dcfr_alternative_form}
The regularizer proposed by \cite{xu2020algorithmic} can be alternatively expressed as:

\begin{equation}
R_{\text{DCFR}} = \sup_{h} Q(h) = \E[ ( \Prob(A=1|f(X),L) - \Prob(A=1|L) )_+ ]
\end{equation}
\end{proposition}


To characterize the connection between $R_{\text{DCFR}}$ and CDP, Proposition~\ref{prop:dcfr_cdd_relationship} shows that when $A$ and $Y$ are binary variables, the relationship between $R_{\text{DCFR}}$ and CDP is dependent on both the rates of $A=1$ and $A=0$ at each level of the legitimate features $L$. The consequence of this is that the relationship between $R_{\text{DCFR}}$ and CDP can be virtually unbounded; in other words, the value of $R_{\text{DCFR}}$ is uninformative to determine CDP, unless $R_{\text{DCFR}} = 0$. 

\begin{proposition} \label{prop:dcfr_cdd_relationship}

Let the sensitive feature$A$, the outcome $Y$ and the model ouput $f(X)$ be binary, and let $\mathcal{X}_+ = \left\{x \in \mathcal{X}: \mathbb{P}(f(X)|A=1) - P(f(X)) > 0 \right\}$. Then, within each level $l$ of the legitimate features $L$ we have that and for $X \in \mathcal{X}_+$:

\begin{equation*}
\frac{\text{CDP}(f(X)|L)}{R_{\text{DCFR}}(f(X)|L)} = \frac{\P(f(X)|L)}{\P(A=0|L)\P(A=1|L)}
\end{equation*}
    
\end{proposition}



\textbf{Illustrative example}. We use the following example to highlight the consequences of Proposition~\ref{prop:dcfr_cdd_relationship}. Let's assume a simple university admission scenario, in which the sensitive feature $A$ is gender and we assume the same level of income $L$:

\begin{tabular}{cc}
\begin{minipage}{0.4\textwidth}
\centering
        \begin{tabular}{@{}lcc@{}}
\toprule
        & Male & Female \\ \midrule
Admitted  & a & b \\
Not Admitted & c & d \\ \bottomrule
\end{tabular}%
\end{minipage}&
\begin{minipage}{0.6\textwidth}
\begin{flushleft}
\begin{equation*}
CDP = \frac{a}{a+c}-\frac{b}{b+d}
\end{equation*}
\begin{equation*}
R_{\text{DCFR}} = \frac{a}{a+b}-\frac{c}{c+d}
\end{equation*}
\end{flushleft}
\end{minipage}
\end{tabular}

In this simple example, reducing CDP implies minimizing the difference in acceptance rate by gender, while reducing $R_{\text{DCFR}}$ implies minimizing the difference between the ratio of admitted males and the proposition of males in the candidate group. Figure \ref{fig:res:Xucomp_simple_example} highlights in practice how the dependency of $R_{\text{DCFR}}$ on the proportion of males makes the value of $R_{\text{DCFR}}$ not informative for CDP. Figure \ref{fig:res:Xucomp_simple_example} (left) shows the different values $R_{\text{DCFR}}$ can attain according to different male proportion in the datasets; the more males the steeper the slope in the CDP - $R_{\text{DCFR}}$ curve. This is particularly problematic as the regularizer averages across different levels of the legitimate feature $L$, where $R_{\text{DCFR}}$ and CDP might have significantly different numerical relationship. During training, the higher values of $R_{\text{DCFR}}$  will have the most importance, but this does not guarantee the highest disparities are being mitigated. Finally, as the relationship varies across many levels (potentially infinitely many of them if $L$ is continuous), makes this phenomenon impossible to control for via hyper-parameter tuning.


\begin{figure}[!htb]
    \centering
    \begin{minipage}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/simple_example_xu/cdd_qh_plot_10k.pdf}
    \end{minipage}%
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figure/simple_example_xu/cdd_fairbit_plot_10k.pdf}
    \end{minipage}
    \caption{\textit{Left}: $Q(h)$ versus conditional demographic disparity (CDD), varying the proportion of females and the acceptance rate of male vs. female in the simple example. In this example we have simulated $10,000$ candidates, and varied CDD by using a hyper-parameter $\delta$, such that $
P(\text{Accept} | \text{Male}) = 0.5 + \delta$ and $P(\text{Accept} | \text{Female}) = 0.5 - \delta.$ Different acceptance rates lead to various levels of CDD and $Q(h)$ values; the proportion of females controls the slope of this CDD-$Q(h)$ curve. More specifically, the fewer the females, the higher the CDD-$Q(h)$ slope, meaning a smaller value of $Q(h)$ would correspond to a much higher CDD. A 1:1 relationship (i.e., a slope of $1$) only happens if the ratio of females to male is 1:1.  }
    \label{fig:res:Xucomp_simple_example}
\end{figure}



\subsection{Modified approaches}


\mg{todo: change language} As discussed above, we are not aware of existing methods designed to target CDP when the legitimate features are discrete with many levels, or continuous. It is therefore not immediately obvious how to choose existing methods that can serve as meaningful points of comparison with our method. We selected two methods, guided by the following observation.

% We note that if $(L, f(X)) \indep A$, then $f(X) \indep A\mid L$ by the weak union property of conditional independence. This observation suggests that 
\begin{remark}\label{remark:weak_union} It follows from the weak union property of conditional independence that if $(L, f(X)) \indep A$, then $f(X) \indep A\mid L$, i.e. conditional demographic parity is satisfied. \label{remark:weak_union}
\end{remark}
Recall that $L \subset X$, and $A \not\subset X$. If the features $X$ are independent of the sensitive feature $A$, then the condition of the remark is trivially satisfied, so CDP is satisfied. Of course, this is not the case in general, but $X$ may be transformed to be orthogonal to $A$. Since the condition $(L, f(X)) \indep A$ is stronger than CDP, it is even harder to satisfy in general, but nevertheless this observation leads to two methods which may effectively target CDP in some circumstances.

\paragraph{Pre-processing repair} This method proposed by Feldman et al. \cite{Feldman2015disparate}\ is a pre-processing method which utilizes a transformation or ``repair'' $X \mapsto \tilde{X}$ such that $\tilde{X}$ is approximately independent of $A$, at least with respect to the empirical measure in the training data. It follows from Remark \ref{remark:weak_union} that $f(\tilde{X})$ is approximately independent of $A$ conditional on $\tilde{L}$. Note that $f(\tilde{X}) \indep A \mid \tilde{L} \centernot\implies f(\tilde{X}) \indep A \mid L$, so this method cannot target CDP in general settings. However, if the transformation $L \mapsto \tilde{L}$ happens to be minimal, then this method may result in approximate CDP. This method includes a \textit{repair level} parameter in $[0, 1]$, where 0 indicates no transformation, 1 indicates the full transformation, and values in between represent degrees of repair.

% In addition to our main approach \bcd~described in Section \ref{section:approach}, we propose an adaptation of an existing fairness method (adversarial debiasing \cite{zhang2018mitigating}), originally designed to target DP, such that it can be used for imposing CDP. Moreover, we discuss conditions under which the pre-processing approach proposed by Feldman et al. \cite{Feldman2015disparate}\ could be effectively used to enforce conditional demographic parity in addition to the originally intended demographic parity. 

\paragraph{Adversarial debiasing } The second method we choose is an in-processing method by Zhang et al. \cite{zhang2018mitigating}, who use adversarial training to target DP (as well as equality of odds and equality of opportunity). In the case of DP, the predictor model is trained to predict the label $Y$ of each sample from the input features $X$, while the adversary is trained to predict the sensitive feature $A$ from the outcome of the predictor $f(X)$. We modify their method to provide the adversary not only with $f(X)$ but also the legitimate features $L$. If the adversary is unable to predict $A$ from $(f(X), L)$, then, by Remark \ref{remark:weak_union}, $f(X)$ will satisfy CDP. Once again, this may happen, but it is not guaranteed to happen in general. Suppose as an extreme example that $L$ is perfectly correlated with $A$. Then the adversary will always be able to predict $A$ regardless of $f(X)$, and CDP will not hold. This approach does not include a parameter to control the fairness-performance trade-off.

% It follows from the weak union property of conditional independence (Remark \ref{remark:weak_union}) that if $(f(X), L) \indep A $ then $f(X) \indep A \mid L$, i.e. we have conditional demographic parity. The main drawback of this approach is that it does not include a parameter to systematically control the performance-fairness tradeoff. %We provide the results for both the original adversarial debiasing algorithm (targeting DP) as well as our adaptation that targets CDP.


\mg{ Adversarial learning will still try to make the marginals of $\hat Y$ as well as conditionals $\hat Y\mid L$ and $L \mid \hat Y$ similar to one another to make it harder for the adversary model to predict $A$ (btw, \bcd\ also tries to minimize all 3). It is true that if $L$ and $A$ are correlated there is a lower bound to its performance, but still achieving that lower bound (which will happen when the adversary relies only on $L$ means achieving CDP.)
}

==> related_work.tex <==
% This section first covers related works in the fairness literature, with a particular focus on optimal transport applications to Fairness. In Section~\ref{sec:DCFR} we compare with DCFR \cite{xu2020algorithmic}, which is the current state of the art for the conditional fairness.

%\paragraph{Algorithmic Fairness} \todo{Fill in} \luhao{Do we need to include some references in CDP?}
\textbf{Demographic and conditional demographic parity}
There are a vast number of methods designed to target demographic parity (see \cite{hort2022BiasMitigation}, Table 9), but very few which are explicitly designed for conditional demographic parity \cite{zliobaite2011HandlingConditionalDiscrimination, kamiran2013QuantifyingExplainableDiscrimination}. (See \cite{hort2022BiasMitigation, pessach2023ReviewFairnessMachine} for recent surveys of fairness definitions and methods. Note that the terms demographic and statistical parity came into usage after some of these methods were developed.) An obvious approach to enforce conditional demographic parity is stratifying on the legitimate or ``explanatory'' feature and applying methods designed to achieve demographic parity within each stratum \cn. In principle, any method for demographic parity can be applied in this way, but this is only feasible when the legitimate feature is discrete with a small number of levels, and it has the disadvantage that the amount of data per level is much smaller than the total sample size. 


By contrast, our method applies a single regularizer to the entire dataset, and it can handle legitimate features that are discrete with many levels or continuous.

In general, fairness methods may be divided into \textit{pre-processing} methods, which transform the training data; \textit{in-processing} methods, which use constraints or regularization terms to guide the model training process; and \textit{post-processing} methods, which learn transformations of existing models. There are dozens or even hundreds of methods in each category, so once again we refer the reader to recent surveys of these methods \cite{hort2022BiasMitigation, pessach2023ReviewFairnessMachine}. Our method is an in-processing approach, since we use a regularizer during model training.

\textbf{Fairness for binary vs. continuous model outputs.}
The majority of the algorithmic fairness literature considers classification settings in which the final model outputs are binary, though there is a growing set of methods that can handle regression settings with continuous model outputs \cite{chzhen2020fair, Romano2020neurips, coston2021CharacterizingFairnessSet, mishler2021FADEFAirDouble}. Many methods which can handle continuous outputs only aim to equalize the first moments of the output distributions across levels of the sensitive feature (e.g. the average loan amount for males vs. females); a smaller but growing number target full equality of the output distributions \cite{chzhen2020fair, Romano2020neurips}. Our method falls in the latter category, aiming to ensure equality of conditional output distributions across levels of the legitimate feature, regardless of whether the output is discrete or continuous. (Note that when the output is binary, equalizing the first moments is equivalent to equalizing the full distributions, since the distribution of a Bernoulli random variable is fully specified by its mean.)

\textbf{Optimal transport for fairness.}
% \paragraph{Optimal transport for fairness.}
Optimal transport has been increasingly used for fairness-related applications, including fair edge prediction, training fair classifiers, and uncovering discrimination in classifiers \cite{black2020fliptest,silvia2020general,laclau2021all,si2021testing,zehlike2020matching,chiappa2021fairness,buyl2022optimal,yang2022obtaining,rychener2022metrizing}. Many methods work by imposing a small optimal transport distances between output distributions, in order to impose (approximate) statistical independence with respect to sensitive features. This allows users to target demographic parity as well as other criteria, whether by pre-processing(\cite{feldman2015certifying,johndrow2019algorithm,gordaliza2019obtaining}), in-processing (\cite{rychener2022metrizing}), or post-processing (\cite{jiang2020wasserstein,chzhen2020fair}) methods. Optimal transport techniques generally require the specification of a distributional distance function. Most papers that apply optimal transport to fairness rely on the \textit{Wasserstein distance}.
% In binary classification problem, \cite{gordaliza2019obtaining} considers repair methods based on the Wasserstein barycenter which yields a trade-off between minimal information loss and a certain amount of fairness.
% \cite{black2020fliptest} produces a ranking of features that are most associated with the model’s behavior on the flipset. \cite{silvia2020general} proposes a general approach to fairness based on transporting distributions corresponding to different sensitive attributes to a common distribution. \cite{laclau2021all} formulates the problem of fair edge prediction, and proposes an embedding-agnostic repairing proce- dure for the adjacency matrix of an arbitrary graph with a trade-off between the group and individual fairness. 
% Some of the literature considers the \textit{distributionally robust optimization} (DRO) to enforce the fairness in training machine learning models, in the sense that their performance is invariant under certain sensitive perturbations to the inputs (\cite{yurochkin2019learning,hashimoto2018fairness,rezaei2019fair}).
As discussed in Section \ref{subsection:bicausal}, the Wasserstein distance is suitable for targeting demographic parity, but not for targeting conditional demographic parity. To target conditional demographic parity, we utilize instead a related but distinct distance known as the \textit{bi-causal transport distance}. This distance does not appear to have been used previously in the context of algorithmic fairness. %, a notion that is related to Wasserstein distance but imposes additional assumption on the transport plan; see Section \ref{section:notation_and_setup} for its definition and a more in-depth discussion.

